Tight homomorphisms and Hermitian symmetric spaces

We introduce the notion of tight homomorphism into a locally compact group with nonvanishing bounded cohomology and study these homomorphisms in detail when the target is a Lie group of Hermitian type. Tight homomorphisms between Lie groups of Hermitian type give rise to tight totally geodesic maps of Hermitian symmetric spaces. We show that tight maps behave in a functorial way with respect to the Shilov boundary and use this to prove a general structure theorem for tight homomorphisms. Furthermore we classify all tight embeddings of the Poincare' disk.

==> kahlerform.tex <==
\section{A Criterion for Tightness}\label{sec_criterion}

Totally geodesic embeddings of
symmetric spaces are in one to one correspondence with Lie algebra
homomorphism respecting the Cartan decompositions.  More precisely,
let now $G_1, G_2$ be Lie groups of Hermitian type, that are connected
semisimple real Lie groups with finite center and no compact factors
such that the associated symmetric spaces $\Xx_j$ are Hermitian. Let
$x_j \in \Xx_j$ be a base point and $K_j = \stab_{G_j}(x_j)$ the
corresponding maximal compact subgroup of $G_j$. Let $\frakg_j=
\frakk_j\oplus \frakp_j$ be the corresponding Cartan decomposition of
the Lie algebra of $G_j$, where $\frakk_j = {\rm Lie} (K_j)$ and
$\frakp_j$ is the orthogonal complement with respect to the Killing
form $\frakB_j$ on $\frakg_j$.  Then every totally geodesic embedding
$f: \Xx_1 \to \Xx_2$, with $f(x_1) = x_2$ induces a Lie algebra
homomorphism $\rho_f: \frakg_1 \to \frakg_2$ which respects the Cartan
decomposition. Conversely every Lie algebra homomorphism $\rho:
\frakg_1 \to \frakg_2$ which respects the Cartan decomposition gives
rise to a totally geodesic embedding $f_\rho: \Xx_1 \to \Xx_2$ with
$f(x_1) = x_2$.  In this section we will obtain a criterion for the
tightness of a totally geodesic embedding $f: \Xx_1\to \Xx_2$ in terms
of the Lie algebra homomorphism $\rho_f$.

For this we will make use of the isomorphism 
\bq\label{eq_homcom}
\hom(\frakk_j, i\RR) \to \Omega^2(\Xx_j)^{G_j} \to \hcb^2(G_j,\RR)\,,
\eq 
where the first map associates to a homomorphism $\lambda \in
\hom(\frakk_j, i\RR)$ the unique $G_j$-invariant differential form on
$\Xx_j$ whose value at $x_j$ is 
\bqn (\omega_\lambda)_{x_j}(X,Y) :=
\frac{1}{4\pi i} \lambda([X,Y])\,, 
\eqn 
for $X,Y \in \frakp_j \cong T_{x_j}\Xx_j$.

%$\Xx_1, \Xx_2$ be symmetric spaces, $G_i = \Is(\Xx_i)^\circ$, $\frakg_i =
%{\rm Lie} (G_i)$ and $\frakg_i = \frakk_i \oplus \frakp_i$ be Cartan
%decomposition associated to the choice of two base points $x_i \in
%\Xx_i$. Then every totally geodesic embedding $f: \Xx_1 \to \Xx_2$,
%$f(x_1) = x_2$ induces a Lie algebra homomorphism $\rho_f: \frakg_1 \to
%\frakg_2$ respecting the Cartan decomposition, conversely every such
%Lie algebra homomorphism $\pi: \frakg_1 \to \frakg_2$ gives rise to a
%totally geodesic embedding $f_\pi: \Xx_1 \to \Xx_2$ with 
%$f(x_1) = x_2$. 

%When the $\Xx_i$ are Hermitian symmetric spaces the Lie algebra
%$\frakk_i$ of the maximal compact subgroup $K_i < G_i$ has a one
%dimensional center $\<Z_i\>\Zz(\frakk_i)$. The relative position of the image of
%$\rho_f(Z_1)$ with respect to $Z_2$ gives a simple criterium 
%for tightness. Namely, a totally geodesic embedding $f: \Xx_1 \to
%\Xx_2$ is tight if and only if $\rho_f(Z_1)$ decomposes 
%as $\pm Z_2 \oplus C \in \Zz(\frakk_2) \oplus \frakk_2^{ss}$, where
%$\frakk_2^{ss}$ denotes the semisimple part of $\frakk_2$. 
%Note that totally geodesic embeddings $\Yy \to \Xx$ between symmetric
%spaces are in one-to-one
%correspondence with homomorphisms of the corresponding Lie algebras
%$\frakh \to \frakg$ preserving the Cartan decomposition. In this
%section we give a criterium for tightness in terms of the
%corresponding Lie algebra homomorphism.
%
%Let $G$ be a group of Hermitian type, that is a connected semisimple real Lie group of
%with finite
%center and no compact factors such that the associated symmetric space
% $\Xx = G/K$ is Hermitian. We fix $G$-invariant complex structure $J$
% on $\Xx$. Let $K<G$ be a maximal compact subgroup, 
%$x_0 = eK \in \Xx$ the $K$-fixed point and $\frakg = \frakk
%\oplus \frakp$ the corresponding Cartan decomposition of the Lie algebra of $G$,
%where $\frakk= {\rm Lie}(K)$ and $\frakp$ its orthogonal complement
%with respect to the Killing from $\frakB$ on $\frakg$. 
%There exists a unique element $Z_\frakg \in \Zz(\frakk)$ in the center
%of $K$ such that $\ad(Z_\frakg)|_\frakp$ gives  the complex
%structure $J$ via the identification $T_{x_0} \Xx \cong \frakp$. 

Fix a $G_j$-invariant complex structure $J_j$ on $\Xx_j$. Then there exists a unique element $Z_j=Z_{\frakg_j} \subset \Zz(\frakk_j)$ in the center of $\frakk_j$ such that $\ad(Z_j)|_{\frakp_j}$ gives the complex
structure $J_j$ via the identification $T_{x_j} \Xx_j \cong \frakp_j$.

The Killing form $\frakB_j$ restricted to $\frakk_j$ is a nondegenerate negative definite symmetric bilinear form. We consider the decomposition, orthogonal with respect to the Killing form, 
\bqn
\frakk_j = \RR Z_j \oplus \Zz(\frakk_j)^{\perp_{Z_j}} \oplus \frakk^{ss}_j\,,
\eqn
where $\Zz(\frakk_j)^{\perp_{Z_j}}$ is the part of the center which is orthogonal with respect to $Z_j$ and $\frakk^{ss}_j$ is the semisimple part of $\frakk_j$. 
We can identify $\RR Z_j \cong i\RR$ by sending $Z_j \to i$. 

Then the orthogonal projection of an element $X \in \frakk_j$ onto $\RR Z_j$ defines a homomorphism 
$\lambda_j \in \hom(\frakk_j, i\RR)$, determined by 
\bqn
X = -i\lambda_j(X) Z_j \oplus C_X \oplus C_S\,, 
\eqn 
where $C_X \in \Zz(\frakk_j)^{\perp_{Z_j}}$ and $C_S\in  \frakk^{ss}_j$.

%\begin{prop}
%The K\"ahler class $\klb = [\omega_{\lambda}]_{\rm b} \in \hcb^2(G,\RR)$ is positive.
%\end{prop}
%\begin{proof}
%ADD PROOF
%\end{proof}
To obtain a criterion for the tightness in terms of the homomorphism $\lambda$ we let 
$\frakg_0= \frakk_0 \oplus \frakp_0$ denote the Lie algebra $\fraks\frakl(2,\RR)$ and $Z_0 \in \frakk_0$ 
the element which defines the standard complex structure on the Poincar\'e disk $\DD$. 
We let $d_j: \DD \to \Xx_j$ with $d_j(0) = x_j$ be a totally geodesic embedding of $\DD$ as a 
tight holomorphic disc in $\Xx_j$.
\begin{prop}\label{prop:criterion}
A totally geodesic embedding $f: \Xx_1 \to \Xx_2$ is tight and positive 
if and only if the Lie algebra homomorphism $\rho_f: \frakg_1 \to \frakg_2$ satisfies  
\bqn
\lambda(\rho_f(\rho_{d_1}(Z_0))) = \lambda(\rho_{d_2}(Z_0))\,, 
\eqn
where $\rho_{d_j}: \frakg_0 \to \frakg_j$ is the Lie algebra
homomorphism corresponding to the tight holomorphic 
embedding $d_j: \DD \to \Xx_i$.
\end{prop}
\begin{proof}
Since the embedding of a tight holomorphic disk is tight and positive,  
Lemma~\ref{lem:composition} implies that the totally geodesic embedding 
$f: \Xx_1 \to \Xx_2$ is tight and positive if and only if $f\circ d_1: \DD \to \Xx_2$ 
is a tight and positive totally geodesic embedding of the disc. 
Thus it suffices to prove that a totally geodesic embedding $f': \DD \to \Xx_2$ is tight and 
positive if and only of $\lambda(\rho_{f'}(Z_0)) = \lambda(\rho_{d_2}(Z_0))$. 
Since $\Omega^2(\DD)^{\SL(2,\RR)} = \RR \omega_\DD$ the forms 
$f'^*\omega_{\lambda} \in \Omega^2(\DD)^{\SL(2,\RR)}$ and
$d_2^*\omega_{\lambda} \in \Omega^2(\DD)^{\SL(2,\RR)}$ are
proportional.  
Moreover since  $\Omega^2(\DD)^{\SL(2,\RR)}\cong \hcb^2(\SL(2,\RR),\RR) = \RR \kappa_{\DD}^{\rm b}$, 
and $d_2: \DD \to \Xx_2$ is a tight and positive embedding, 
the embedding $f'$ is tight if and only if the constant of
proportionaliy between $f'^*\omega_{\lambda}$ and
$d_2^*\omega_{\lambda}$ is one, but this constant is equal to
$\frac{\lambda(\rho_{f'}(Z_0))}{
  \lambda(\rho_{d_2}(Z_0))}$.\marginpar{polish proof}
\end{proof} 

With the following Lemma, Proposition~\ref{prop:criterion} takes on very simple form when 
$\Xx_1$ and $\Xx_2$ are of tube type.
\begin{lemma}\cite[Proposition~3.12.]{Koranyi_Wolf_65_annals}\label{lem:tubetype}
A Hermitian symmetric space $\Xx_j$ is of tube type 
if and only if there exists an embeddings of a tight holomorphic disc $d_j:\DD \to \Xx_j$ with 
$\rho_{d_j}(Z_0) = Z_j$.
\end{lemma}
%We now assume that $\Xx$ is irreducible, then center $\Zz(\frakk)$ is
%one dimensional and the Lie algebra $\frakk$ decomposes as 
%\bqn
%\frakk= \Zz(\frakk)\oplus \frakk^{ss},
%\eqn 
%where $\frakk_{ss}$ is the
%Lie algebra of the semisimple part of $K$. 
%
%The center $\Zz(\frakk)$ composes further into the direct sum of $\RR Z_\frakg$ and the orthogonal 
%complement $\Zz_\frakg^\perp$ with respect to the Killing $\frakB_{|_\frakk}$.

\begin{cor}\label{tight_tight}
Let $\Xx_1$ and $\Xx_2$ be Hermitian symmetric spaces of tube type. A
totally geodesic embedding $f: \Xx_1 \to \Xx_2$ is tight and positive
if and only if  
the corresponding Lie algebra homomorphism $\rho_f: \frakg_1 \to \frakg_2$ satisfies 
\bqn
\lambda(\rho_f(Z_1)) = 1\,.
\eqn
\end{cor}
\begin{proof}
Let $\rho_{d_j}: \frakg_0 \to \frakg_j$ be the Lie algebra homomorphism corresponding to the embedding of a 
tight holomorphic disc with $\rho_{d_j}(Z_0) = Z_j$ (see Lemma~\ref{lem:tubetype}). 
Since $\lambda(\rho_f(Z_1)) = \lambda(\rho_f(\rho_{d_1}(Z_0)))$ and $\lambda(\rho_{d_2}(Z_0)) = \lambda(Z_2)= 1$ 
Proposition~\ref{prop:criterion} implies the claim. 
\end{proof}
%
%For any $X\in \frakk$ 
%there exists a unique $\lambda_{Z_\frakg}(X)  \in\RR$ such that 
%\bqn
%X= \lambda_{Z_\frakg}(X) Z_\frakg \, \mod  \frakk^{ss}.
%\eqn
%
%Since $[\frakp,\frakp]\subset \frakk$  
%\bqn
%\Lambda_{Z_\frakg}(V,W):=\lambda_{Z_\frakg}([V,W]) \quad \text{ for all }V,W\in\frakp.
%\eqn 
%is a nondegenerate skew-symmetric $K$-invariant bilinear form on
%$\frakp$. 
%
%We denote by $\Omega_{Z_\frakg} \in \Omega^2(\Xx)^G$  
%the unique $G$-invariant
%real 2-form whose value at $x_0$ is 
%\bqn
%(\Omega_{Z_\frakg})_{x_0}(V,W) :=
%\frac{1}{4\pi}\lambda_{Z_\frakg}([V,W]), 
%\eqn
%and by $c_{\Omega_Z}: G\times G \times G \to \RR$, $(g_0, g_1,
%g_2)\mapsto
%\int_{\Delta(g_0 x_0, g_1 x_0, g_2 x_0)}
%\Omega_{Z_\frakg}$ the corresponding (bounded) cocycle. 
%Note that the associated bounded K\"ahler class $\kZb = [c_{\Omega_Z}]_b \in
%\hcb^2(G,\RR)$ is positive, so that, in virtue of
%Proposition~\ref{prop:positive}, 
%we can use $\kZb$ instead of $\kgjb$ so investigate
%tight embeddings.
%
%\subsection{Criterion for Tightness}
%The following criterion will be useful to classify tight embeddings in \S~\ref{sec:classification}.
%\begin{prop}\label{tight_tight}
%Let $G_1, G_2$ be of Hermitian type and of tube type and $\frakg_1,
%\frakg_2$ their Lie algebras. Assume that $G_2$ is (almost) simple.  
%A continuous homomorphism $\rho: G_1 \to G_2$ is tight if an only if the induced homomorphism 
%$\rho_*: \frakg_1 \to \frakg_2$ of Lie algebras satisfies 
%\bqn
%|\lambda_{\frakg_2}(\rho_*(Z_{\frakg_1}))| = 1.
%\eqn
%\end{prop}
%Before the continue to give the proof, let us recall that 
%\begin{prop}\cite[Proposition~3.12.]{Koranyi_Wolf_65_annals}
%A Lie group $G$ of Hermitian type is of tube type if and only if
%there exists a three dimensional simple subalgebra  $\frakl \subset 
%\frakg$ with $Z_\frakg\subset\frakl$.
%\end{prop}
%Note that the orbit $\exp(\frakl)x_0$ of this three dimensional simple
%subalgebra is a tight holomorphic disk in
%$\Xx$. Up to conjugation  
%the Lie algebra homomorphism $D_*: \fraks\frakl(2,\RR) \to
%\frakl\subset \frakg$ 
%correponding to the homomorphism $D: \SL(2,\RR) \to G$ associated to 
%an embedding of a tight holomorphic disk $d: \DD \to \Xx$ 
%satisfies 
%$D_*(Z_{\fraks\frakl(2,\RR)})=Z_\frakg$.  
%In particular, we have
%$\lambda_\frakg(D_*(Z_{\fraks\frakl(2,\RR}))= 1$ and therefore
%$D^* \kZgb = \kZsb$.  
%And, since $\kZgb$ is positive we get
%\begin{lemma}\label{lem:tight_sl}
%A homomorphism $\rho: \SL(2,\RR) \to G$ is tight and positive 
%if and only if 
%\bqn
%{\rho}_* \kZgb = \kZsb.
%\eqn
%\end{lemma} 
%\begin{proof}[Proof of Proposition~\ref{tight_tight}]
%It suffices to show that $\rho: G_1 \to G_2$ is tight and positive if
%and only if $\lambda_{\frakg_2}(\rho_*(Z_{\frakg_1}) = 1$ 
%
%Consider first the case when $\frakg_1 = \fraks\frakl(2,\RR)$, then
% $\rho^*\kZgtb=\kZsb$ if and only if 
% and $\lambda_{Z_\frakg}([\rho_*(X_1),\rho_*(Y_1)]) =
% \lambda_{Z_{\fraks\frakl(2,\RR)}}([X_1,Y_1])$ for all  
%$X_1, Y_1 \in \frakp_{\fraks\frakl(2,\RR)}$. Taking $X_1, Y_1$ to be
% the basis of $\frakp_{\fraks\frakl(2,\RR)}$  
%with $[X_1, Y_1] = Z_{\fraks\frakl(2,\RR)}$, this is the case if and only if 
%\bqn
%\lambda_{Z_{\frakg_2}}(\rho_*(Z_{\fraks\frakl(2,\RR)})) &=&
% \lambda_{Z_{\frakg_2}}(\rho_*([X_1,Y_1]))\\ 
%&=& \lambda_{Z_{\frakg_2}}([\rho_*(X_1),\rho_*(Y_1)]) \\
%&=& \lambda_{Z_{\fraks\frakl(2,\RR)}}([X_1,Y_1]) \\
%&=&\lambda_{Z_{\fraks\frakl(2,\RR)}}(Z_{\fraks\frakl(2,\RR)}) \\
%&=& 1. 
%\eqn

%For the general case, let $L= \SL(2,\RR)$ and $D_*: L\to G_1$ be a tight
% homomormphism corresponding to an embedding of a tight holomorphic disk.  
%Note that, by Lemma~\ref{lem:composition}, $\rho: G_1\to G_2 $ is
% tight and positive if and only if 
%$\rho\circ D: L \to G_2$ is tight and positive. 
%By the above we have that $\rho\circ D: L \to G_2$ is
% tight and positive if and only if  
%\bqn
%\lambda_{Z_{\frakg_2}} ((\rho\circ D)_* (Z_{\frakl}) = 1.
%\eqn 
%This togehter with 
%\bqn
%\lambda_{Z_{\frakg_2}} ((\rho\circ D)_* (Z_{\frakl}))
%& = &\lambda_{Z_{\frakg_2}}(\rho_*(D_* (Z_{\frakl}))\\
%&=& \lambda_{Z_{\frakg_2}}(\rho_*(Z_{\frakg_1})).
%\eqn
%implies the claim.
%\end{proof}
%
%In a slightly modified way the above criterion applies to tight
%embeddings of Hermitian symmetric spaces that are not of tube type. 
%Let $f:\Yy\to \Xx$ be a tight totally geodesic embedding of Hermitian
%symmetric spaces. The embedding $f:\Yy\to \Xx$ is tight if and only if the restriction
%to the maximal symmetric subspace of tube type $\Tt_\Yy$ in $\Yy$ is
%tight.
%Since the embedding of a maximal subdomain of tube type $\Tt_\Xx$
%in $\Xx$ is tight, the Lie algebra homomorhism $\rho_*: \frakh\to \frakg$ 
%corresponding to a tight embedding $f:\Yy \to \Xx$ has to satisfy
%$\lambda(\rho_*(Z_{\Tt_\Yy}))  = \lambda(Z_{\Tt_\Xx})$.
%The constant $c$ is not universal
%but depends on $\Xx$. 

We compare the tightness criterion with the characterizations of Lie
algebra homomorphism corresponding to  
holomorphic totally geodesic embeddings. 
Recall the following definitions from \cite{Satake_book}:

\begin{defi}
Suppose $\frakg_1, \frakg_2$ are simple Lie algebras of Hermitian type. 
Then a homomorphism $\rho:\frakg_1\to \frakg_2$ is said to be of type 
\begin{enumerate}
\item[$(\h1)$] if $\ad(\rho(Z_1))= \ad(Z_2)$.
\item[$(\h2)$] if $\rho(Z_1)=Z_2$.
\item[$({\h2}^\prime)$] if $\rho$ is $(\h1)$ and the induced $\CC$-linear 
map $\Dd_1\to \Dd_2$ maps the Shilov boundary 
into the Shilov boundary.
\end{enumerate}
\end{defi}

Lie algebra homomorphisms of type $(\h1)$ are in one-to-one
correspondence with holomorphic totally geodesic embeddings $\Xx_1 \to \Xx_2$. 
Theorem~\ref{thm:tight_embedding_one} implies

\begin{cor}
Assume that $f:\Xx_1\to \Xx_2$ is a holomorphic tight embedding. Then the corresponding Lie algebra 
homomorphism $\rho_f: \frakg_1\to \frakg_2$ is a $(\h2^\prime)$ homomorphism.
\end{cor}

Lemma~\ref{tight_tight} together with results of Satake
\cite[Proposition~10.12]{Satake_book} implies the following

\begin{cor}\label{H2_hom}
Suppose $\Xx_1, \Xx_2$ are Hermitian symmetric spaces of tube type. 
Then $f:\Xx_1\to \Xx_2$
is a tight and holomorphic embedding if and only if the 
corresponding homomorphism of Lie algebras 
$\rho_f:\frakg_1\to \frakg_2$ is an $(\h2)$-homomorphism, that is if 
$\rho_f(Z_1)=Z_2$.
\end{cor}

\begin{rem}
When $\frakg_1, \frakg_2$ are not of tube type, the property of being an
$(\h2)$-Lie algebra homomorphism does not imply tightness. For
$\fraks\fraku(1,n) = \aut(V,h)$ the representations of $\fraks\fraku(1,n)$  
on $\Lambda^k(V)$ preserving the Hermitian form induced 
by $h$ are always $(\h2)$ \cite[page 188]{Satake_book}, but as we will
see below they are tight only for $k=1$. 
\end{rem}

\subsection{Examples and Non-Examples}\label{sec:examples}
% in order 
%to illustrate this class of totally geodesic embeddings.\\
By Corollary~\ref{H2_hom} $(\h2)$ Lie algebra homomorphisms 
give tight holomorphic embeddings if the Hermitian symmetric spaces are of tube type. 
All $(\h_2)$ Lie algebra were classified by Satake \cite{Satake_annals} and Ihara \cite{Ihara_65, Ihara_66}. 
%This give the list of the following holomorphic tight embeddings $f: \Xx_1 \to \Xx_2$ 
%among Hermitian symmetric spaces of tube type 
%\marginpar{ put table}
%%\bigskip
%\begin{tabular}{l|l}
%\hline\hline
%{\bf \frakg_1}& {\bf \frakg_2}\\
%\hline\hline
%\frak& {\bf \frakg_2}\\
%\hline\hline
%{\bf \frakg_1}& {\bf \frakg_2}\\
%\hline\hline
%{\bf \frakg_1}& {\bf \frakg_2}\\
%\hline\hline
%\end{tabular}
%\bigskip
\begin{rem}
If we are actually interested in the existence of tight homomorphism of Lie groups of Hermitian type 
the problem gets a bit more complicated, since the Lie algebra homomorphism might only lift to a 
Lie group homomorphism of a finite cover of the adjoint Lie group. 
Satake showed in \cite{Satake_annals} (see also  \cite[Ch.~IV]{Satake_book}) 
that some of the above $(\h2)$ Lie algebra homomorphism lift to Lie group 
  homomorphisms, for example  
\bqn
&\tau:& \SU(n,n) \to \Sp(4n, \RR)\\
&\tau:& \SO^*(4n) \to \Sp(8n,\RR)\\
&\tau:& \Spin(2,n) \to \Sp(2m, \RR), \text{ where $m$ depends on }n\mod 8\,.
\eqn
\end{rem} 
%\bigskip
%An example is the embedding corresponding to the Lie algebra homomorphism 
%$\fraks\fraku(n,n) \to \fraks\frakp(4n,\RR)$ defined by 
%\bqn
%g=\begin{pmatrix} X_{11} & X_2 \\ X_2^* & X_{12} \end{pmatrix}
%\to \begin{pmatrix} A & B \\ \ol{B} & \ol{A} \end{pmatrix}, 
%\eqn 
%with 
%\bqn
%A=\begin{pmatrix} \ol{X_{12}} & 0 \\ 0 & X_{11} \end{pmatrix}\\
%B=\begin{pmatrix} 0 & X_2^T \\ \ol{X_2} & 0 \end{pmatrix}.
%\eqn
%\marginpar{add example Spin, SO*}
%\item Embeddings of maximal 
%subdomains of tube type are tight, for example 
%$\fraks\fraku(n,n) \to \fraks\fraku(n,m)$ with $m>n$.\marginpar{add
%  exceptional example}

An important and interesting tight embedding that is not holomorphic is the embedding of the Poincar\'e disk into the Siegel upper half space obtained 
from the 2n-dimensional irreducible representation $\fraks\frakl(2,\RR) \to \fraks\frakp(2n,\RR)$. 
\begin{prop}\label{irreducible_rep}
The homomorphism $\rho:\fraks\frakl(2,\RR)\to
\fraks\frakp(2n,\RR)$ given by the 
$2n$-dimensional irreducible representation of $\fraks\frakl(2,\RR)$ is tight.
\end{prop}
\begin{proof}
We only have to determine $\lambda(\rho(Z_{\fraks\frakl(2,\RR)}))$, 
given by  
\bqn
\rho(Z_{\fraks\frakl(2,\RR)})=
\lambda(\rho(Z_{\fraks\frakl(2,\RR)}))Z_{\fraks\frakp(2n,\RR)} 
\mod \frakk^{ss}\,, 
\eqn
where $Z_{\fraks\frakl(2,\RR)}$ and $Z_{\fraks\frakp(2n,\RR)}$ are
  generators of the center of the maximal compact Lie subalgebras in
  $\fraks\frakl(2,\RR)$ and $\fraks\frakp(2n,\RR)$ respectively.
For this let $V^{2n}$ the vector space of homogeneous polynomials of degree $n$ in two variables $x,y$, with 
a basis is given by $(P_0, \dots P_m)$, $m= 2n-1$, where $P_k(x,y)= x^{m-k}y^k$. 
The $2n$-dimensional 
irreducible representation of $\fraks\frakl(2,\RR)$ is given by the following action: 
Let $X=\begin{pmatrix} a & b \\ c & -a \end{pmatrix} \in \fraks\frakl(2,\RR)$, then 
\bqn
\rho(X) P_k(x,y)= a(m-2k) P_k + b(m-k) P_{k+1} + c k P_{k-1}\,.
\eqn
This action preserves the skew symmetric bilinear form $\langle .,.\rangle$ on $V$, 
defined by $\langle P_k, P_{m-k}\rangle = (-1)^k {{m}\choose{k}}^{-1}$ 
and gives rise to the irreducible representation 
\bqn
\rho:\fraks\frakl(2,\RR) \to \fraks\frakp(2n,\RR)\,,
\eqn 
into the Lie algebra of the symplectic group ${\rm Sp}(V^{2n},\langle .,.\rangle)$.
The map $J$ defined by $J P_k= (-1)^k P_{m-k}$ gives a complex
structure on $V$ and the element in the center of 
$\frakk\subset \fraks\frakp(2n,\RR)$ which induces the complex structure 
on $\frakp\subset \fraks\frakp(2n,\RR)$ via the adjoint action is $Z_{\fraks\frakp(2n,\RR)}
:=\frac{1}{2} J$.

The image of the element 
\bqn
Z_{\fraks\frakl(2,\RR)} = \frac{1}{2} \begin{pmatrix} 0 & -1 \\ 1 & 0\end{pmatrix}
\eqn
is given by 
$\rho(Z_{\fraks\frakl(2,\RR)}) P_k = \frac{1}{2}((k-m)P_{k+1} + k P_{k-1})$. 
Decomposing $\rho(Z_{\fraks\frakl(2,\RR)})=
\lambda(\rho(Z_{\fraks\frakl(2,\RR) }))Z_{\fraks\frakp(2n,\RR)} \mod \frakk^{ss}$, 
we get 
\bqn
Z_{\fraks\frakp(2n,\RR)}  \rho(Z_{\fraks\frakl(2,\RR)}) = \frac{-\lambda}{4} \id_V \mod Z_{\fraks\frakp(2n,\RR)} \frakk^{ss}\,.
\eqn
Since $\tr (Z_{\fraks\frakp(2n,\RR)} \frakk^{ss})= 0$, 
we have that $\tr(Z_{\fraks\frakp(2n,\RR)}  \rho(Z_{\fraks\frakl(2,\RR)})) = \frac{-\lambda}{4} dim(V)$. 
Now $Z_{\fraks\frakp(2n,\RR)}  \rho(Z_{\fraks\frakl(2,\RR) }) P_k = \frac{1}{4} (-1)^{k+1} [(m-k) P_{m-k-1}- k P_{m-k+1}]$. 
Thus the diagonal terms are $\frac{1}{4} (-1)^{n} (2n-1-n+1)$ for $k={n-1}$,
and $\frac{1}{4} (-1)^n n$  for $k=n$.
Hence 
\bqn
|\tr(Z_{\fraks\frakp(2n,\RR)}  \rho(Z_{\fraks\frakl(2,\RR) }))| =
\frac{n}{2} =\frac{1}{4} dim(V)=|\tr(Z_{\fraks\frakp(2n,\RR)}
Z_{\fraks\frakp(2n,\RR)})|\,, 
\eqn 
and $|\lambda|=1$.
\end{proof}

%\subsubsection{Non-Examples}
%We give also some Non-Examples:
%\begin{notation*}
%A $p\times q$ 
%matrix consisting of a $p \times p$ matrix and $q-p$ zero columns 
%of a $q \times q$ matrix and $p-q$ zero lines, will be denoted by 
%$(A,0)$.
%\end{notation*}
Let us give also some examples of Lie algebra homomorphisms which the reader might think are tight, but which are not.

\begin{prop}\label{prop:irred_not_tight} The irreducible representation $\rho: \fraks\fraku(1,2) \to
   \fraks\fraku(2,4)$ is not tight.
\end{prop}
\begin{proof}
Let $V$ be a $3$-dimensional complex vector space with Hermitian form
of signature $(1,2)$.  
The irreducible representation $\rho: \fraks\fraku(1,2) \to
   \fraks\fraku(2,4)$ is the representation given by the action of
   $\fraks\fraku(1,2)$ on $\sym^2(V)$ with the induced Hermitian form.
Let $Z_{\fraks\fraku(2,4)}$ be the generator of the center of the maximal compact subalgebra on
$\fraks\fraku(2,4)$ and $Z_{\fraks\fraku(2,2)}$ the generator of the center of the maximal compact subalgebra
of the tightly embedded subalgebra $\fraks\fraku(2,2)\subset
\fraks\fraku(2,4)$. Then
$\tr(Z_{\fraks\fraku(2,4)}Z_{\fraks\fraku(2,2)})=-1$, so the
representation $\rho: \fraks\fraku(1,2) \to 
   \fraks\fraku(2,4)$ is tight if and only if 
$|\tr(Z_{\fraks\fraku(2,4)} \rho(Z_{\fraks\fraku(1,1)}))| =
   1$, where $Z_{\fraks\fraku(1,1)}$ is a generator of the center of  
the maximal 
compact subalgebra of $\fraks\fraku(1,1) \subset \fraks\fraku(1,2)$.
Direct computation show that $|\tr(Z_{\fraks\fraku(2,4)} \rho(Z_{\fraks\fraku(1,1)}))| = \frac{1}{6}$, thus $\rho$ is not tight. \marginpar{check the precise value again}
\end{proof}

Regarding a complex vector space $V_\CC$ of dimension $(1+n)$ with a Hermitian form of signature$(1,n)$ as 
real vector space $V_\RR$ of dimension $(2+n)$ with a quadratic form of signature $(2,n)$ provides a 
natural embedding ${\rm SU}(1,n)\to {\rm SO}(2,2n)$. 
The corresponding embedding $\Hh_\CC^n \to \Xx_{2,2n}$ is holomorphic
but it is not tight. 
Since $\Hh_\CC^n$ is of rank one, the totally geodesic embedding extends 
continuously to a map of the boundary of $\Hh_\CC^n$, but its image 
does not lie in the Shilov boundary of $\Xx_{2,2n}$.
%The image of the tight holomorphic disc 
%\bqn
%\begin{pmatrix} 0 & (z,0) \\ (z,0) & 0\end{pmatrix}
%\eqn  
%is  
%\bqn
%\begin{pmatrix} 0 & (Z,0) \\ (Z^T,0) & 0\end{pmatrix}
%\eqn 
%with $Z=\begin{pmatrix} x & y\\ -y & x\end{pmatrix}$, where $x+iy=z$ but the tight holomorphic disc in 
%${\rm SO}(2,2n)$ is given by 
%\bqn
%\begin{pmatrix} 0 & (A,0) \\ (A^T,0) & 0\end{pmatrix},
%\eqn where $A=Z=\begin{pmatrix} a_1 & b_1\\ 0 & 0\end{pmatrix}$.\\
%
%, but in 
%the $\Ad(K)$-orbit of $o_1$.

Tightness indeed depends 
on the complex structure.
% and cannot be reduced to the property 
%that the totally geodesic map extends to the Shilov boundary. 
%This can be illustrated by the following example:
In ${\rm SL}(4,\RR)$ 
there are two copies of ${\rm Sp}(4, \RR)$
\bqn
{\rm Sp}(4, \RR)_A :=\{ g \in {\rm SL}(4,\RR) \,|\, g^* J g = J\}\\
{\rm Sp}(4, \RR)_B :=\{ g \in {\rm SL}(4,\RR) \,|\, g^* \tilde{J} g = \tilde{J}\}\,, 
\eqn
where $J= \begin{pmatrix} 0 & \id\\ -\id & 0 \end{pmatrix}$ and 
$\tilde{J}=\begin{pmatrix} 0 & \Lambda \\ -\Lambda & 0\end{pmatrix}$ 
with $\Lambda=\begin{pmatrix} 0 & 1\\ 1 & 0\end{pmatrix}$,  
which are conjugare by $s= \begin{pmatrix} \id & 0 \\ 0 & \Lambda\end{pmatrix}$. 
%satisfies $ \tilde{J}= sJs^{-1}$ 
%and thus conjugates $s^{-1} {\rm Sp}(4, \RR)_B s={\rm Sp}(4, \RR)_A$.
%
The two embeddings $i_{A,B}: {\rm SL}(2,\RR) \to {\rm SL}(4,\RR)$  
\bqn
i_A\left( \begin{pmatrix} a & b\\ c & d\end{pmatrix}\right) = \begin{pmatrix} a\id
  & b\id \\ c\id & d\id \end{pmatrix}
\eqn

\bqn
i_B\left( \begin{pmatrix} a & b\\ c & d\end{pmatrix}\right) = \begin{pmatrix} a\id
  & b\Lambda \\ c\Lambda & d\id \end{pmatrix}\,.
\eqn
are also conjugate by $s$. 
The image of ${\rm SL}(2,\RR)$ under these two embeddings lie in 
${\rm Sp}(4, \RR)_A \cap {\rm Sp}(4, \RR)_B$. 
The embedding $i_A$ is tight and positive with respect to ${\rm Sp}(4, \RR)_A$ 
but totally real with respect to ${\rm Sp}(4, \RR)_B$.
%, 
%whereas the embedding $i_B$ is tight with respect to ${\rm Sp}(4, \RR)_B$ 
%and totally real with respect to ${\rm Sp}(4, \RR)_A$. 
The boundary $S^1$ of $\DD$ is mapped under both embeddings 
into the Shilov boundaries 
$\cs_A$ respectively $\cs_B$. 
The totally real embedding 
extends to an embedding of ${\rm SL}(2,\CC)$ 
whereas the tight embedding extend to an embedding of ${\rm SO}(2,2)$ into 
${\rm Sp}(4, \RR)$ .
%This example can easily be extended to ${\rm Sp}(2n, \RR)$ to give
%examples of totally geodesic embeddings of the disc $\DD$ which are not tight, 
%neither holomorphic nor totally real, 
%but extend to the Shilov boundary.
\marginpar{Precomposing with a hyperbolization we get thus e.g. two
  representations which are equivalent as SL(4,R) representation, but
  not as Sp(4,R) representations.}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tight"
%%% End: 


!DSPAM:4696a1d5189941140720403!


==> macros.tex <==
%%%%%%%%%% Definitionen von Umgebungen %%%%%%%%%%%%%%%%%%%%%%%%

\newtheoremstyle{mytheorem}% name
  {}%      Space above, empty = `usual value'
  {}%      Space below
  {\slshape}% Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\scshape}% Thm head font
  {.}%        Punctuation after head
  { }%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}% Thm head spec

\newtheoremstyle{mydefinition}% name
  {}%      Space above, empty = `usual value'
  {}%      Space below
  {\upshape}% Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\scshape}% Thm head font
  {.}%        Punctuation after thm head
  { }%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}% Thm head spec

\theoremstyle{mytheorem}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{prop}[lemma]{Proposition}
\newtheorem*{prop*}{Proposition}
\newtheorem{prop_intro}{Proposition}
\newtheorem{cor}[lemma]{Corollary}
\newtheorem{cor_intro}[prop_intro]{Corollary}
\newtheorem{thm}[lemma]{Theorem}
\newtheorem{thm_intro}[prop_intro]{Theorem}
\newtheorem*{thm*}{Theorem}
\theoremstyle{mydefinition}
\newtheorem{rem}[lemma]{Remark}
\newtheorem*{rem*}{Remark}
\newtheorem{rem_intro}[prop_intro]{Remark}
\newtheorem{rems_intro}[prop_intro]{Remarks}
\newtheorem*{notation*}{Notation}
\newtheorem*{warning*}{Warning}
\newtheorem{rems}[lemma]{Remarks}
\newtheorem{defi}[lemma]{Definition}
\newtheorem*{defi*}{Definition}
\newtheorem{defi_intro}[prop_intro]{Definition}
\newtheorem{defis}[lemma]{Definitions}
\newtheorem{exo}[lemma]{Example}
\newtheorem{exos}[lemma]{Examples}
\newtheorem{pp}[lemma]{Properties}
%\newtheorem*{examp*}[lemma]{Example}
\newtheorem{exo_intro}[prop_intro]{Example}
\newtheorem{exos_intro}[prop_intro]{Examples}

\numberwithin{equation}{section}

\newcommand{\bqn}{\begin{eqnarray*}}
\newcommand{\eqn}{\end{eqnarray*}}
\newcommand{\bq}{\begin{eqnarray}}
\newcommand{\eq}{\end{eqnarray}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\ba}{\begin{aligned}}
\newcommand{\ea}{\end{aligned}}


\newcommand{\bibURL}[1]{{\unskip\nobreak\hfil\penalty50{\tt#1}}}

\def\ti{-\allowhyphens}
\newcommand{\thismonth}{\ifcase\month % case 0 --- impossible!
  \or January\or February\or March\or April\or May\or June%
  \or July\or August\or September\or October\or November%
  \or December\fi}
\newcommand{\thismonthyear}{{\thismonth} {\number\year}}
\newcommand{\thisdaymonthyear}{{\number\day} {\thismonth} {\number\year}}
%
%
%
%%%%%%%%%%%%%%%%ù Definitionen von Symbolen %%%%%%%%%%%%%%%%%%%%%%ù

\renewcommand{\AA}{{\mathbb A}}
\newcommand{\BB}{{\mathbb B}}
\newcommand{\CC}{{\mathbb C}}
\newcommand{\DD}{{\mathbb D}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\KK}{{\mathbb K}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\TT}{{\mathbb T}}
\newcommand{\ZZ}{{\mathbb Z}}

\newcommand{\Aa}{{\mathcal A}}
\newcommand{\Bb}{{\mathcal B}}
\newcommand{\Cc}{{\mathcal C}}
\newcommand{\Dd}{{\mathcal D}}
\newcommand{\Ee}{{\mathcal E}}
\newcommand{\Ff}{{\mathcal F}}
\newcommand{\Hh}{{\mathcal H}}
\newcommand{\Ii}{{\mathcal I}}
\newcommand{\Jj}{{\mathcal J}}
\newcommand{\Kk}{{\mathcal K}}
\newcommand{\Ll}{{\mathcal L}}
\newcommand{\Mm}{{\mathcal M}}
\newcommand{\Nn}{{\mathcal N}}
\newcommand{\Oo}{{\mathcal O}}
\newcommand{\Qq}{{\mathcal Q}}
\newcommand{\Pp}{{\mathcal P}}
\newcommand{\Rr}{{\mathcal R}}
\newcommand{\Ss}{{\mathcal S}}
\newcommand{\Tt}{{\mathcal T}}
\newcommand{\Vv}{{\mathcal V}}
\newcommand{\Xx}{{\mathcal X}}
\newcommand{\Yy}{{\mathcal Y}}
\newcommand{\Zz}{{\mathcal Z}}

\newcommand{\fraka}{{\mathfrak a}}
\newcommand{\frakc}{{\mathfrak c}}
\newcommand{\frake}{{\mathfrak e}}
\newcommand{\frakg}{{\mathfrak g}}
\newcommand{\frakh}{{\mathfrak h}}
\newcommand{\frakk}{{\mathfrak k}}
\newcommand{\frakl}{{\mathfrak l}}
\newcommand{\frakm}{{\mathfrak m}}
\newcommand{\frakn}{{\mathfrak n}}
\newcommand{\frako}{{\mathfrak o}}
\newcommand{\frakp}{{\mathfrak p}}
\newcommand{\frakq}{{\mathfrak q}}
\newcommand{\frakr}{{\mathfrak r}}
\newcommand{\fraks}{{\mathfrak s}}
\newcommand{\frakt}{{\mathfrak t}}
\newcommand{\fraku}{{\mathfrak u}}

\newcommand{\frakpp}{{\mathfrak p_+}}
\newcommand{\frakpm}{{\mathfrak p_-}}
\newcommand{\frakkc}{{{\mathfrak k}_\CC}}
\newcommand{\frakgc}{{{\mathfrak g}_\CC}}
\newcommand{\frakpc}{{{\mathfrak p}_\CC}}
\newcommand{\frakB}{{\mathfrak B}}

\newcommand{\tk}{{\tt k}}

\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\sign}{\operatorname{sign}}
%\newcommand{\graph}{\operatorname{graph}}
\newcommand{\aut}{\operatorname{Aut}}
\newcommand{\Int}{\operatorname{Int}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Is}{\operatorname{Is}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\PU}{\operatorname{PU}}
\newcommand{\mo}{\operatorname{mod}}
\newcommand{\ko}{\operatorname{k}}
\newcommand{\Image}{\operatorname{Image}}
\newcommand{\Lie}{\operatorname{Lie}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\esssup}{\operatorname{ess\,sup}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\length}{\operatorname{length}}
\newcommand{\rad}{\operatorname{Rad}}
\newcommand{\essgr}{\operatorname{Ess\,Gr}}
\newcommand{\essim}{\operatorname{Ess\,Im}}
\newcommand{\QHB}{{\operatorname{QH}_\Bb}}
\newcommand{\QHch}{{\operatorname{QH}_\mathrm{c}^\mathrm{h}}}


\renewcommand{\a}{\alpha}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\renewcommand{\L}{\Lambda}
\renewcommand{\l}{\lambda}
\newcommand{\T}{{\rm T}}

\newcommand{\dD}{{\mathbf D}}
\newcommand{\gG}{{\mathbf G}}
\newcommand{\hH}{{\mathbf H}}
\newcommand{\pP}{{\mathbf P}}
\newcommand{\lL}{{\mathbf L}}
\newcommand{\qQ}{{\mathbf Q}}
\newcommand{\nN}{{\mathbf N}}
\newcommand{\uU}{{\mathbf U}}
\newcommand{\vV}{{\mathbf V}}
\newcommand{\wW}{{\mathbf W}}


\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}

\def\ol{\overline}

\def\h{{\rm H}}
\def\hb{{\rm H}_{\rm b}}
\def\ehb{{\rm EH}_{\rm b}}
\def\ha{{\rm H}_{(G,K)}}
\def\hc{{\rm H}_{\rm c}}
\def\hh{{\rm {\widehat H}}}
\def\hhc{{\rm {\widehat H}}_{\rm c}}
\def\hcb{{\rm H}_{\rm cb}}
\def\hhcb{{\rm {\widehat H}}_{\rm cb}}
\def\hhb{{\rm {\widehat H}}_{\rm b}}
\def\ehbc{{\rm EH}_{\rm cb}}
\def\linfty{L^\infty}
\def\linftyw{L^\infty_{\rm w*}}
\def\linftya{L^\infty_{\mathrm{w*,alt}}}
\def\cba{\mathrm{C}_{\mathrm{b,alt}}}
\def\la{L^\infty_{\mathrm{alt}}}
\def\cb{{\rm C}_{\rm b}}
\def\tb{\mathrm{t}_\mathrm{b}}
\def\Tb{\mathrm{T}_\mathrm{b}}
\def\binfty{\mathcal B^\infty_{\mathrm alt}}

\def\one{\mathbf{1\kern-1.6mm 1}}
\def\sous#1#2{{\raisebox{-1.5mm}{$#1$}\backslash \raisebox{.5mm}{$#2$}}}
\def\rest#1{{\raisebox{-.95mm}{$\big|$}\raisebox{-2mm}{$#1$}}}
\def\homeo#1{{\sl H\!omeo}^+\!\left(#1\right)}
\def\thomeo#1{\widetilde{{\sl \!H}\!omeo}^+\!\left(#1\right)}
\def\bu{\bullet}
\def\weak{weak-* }
\def\property{\textbf{\rm\textbf A}}
\def\cont{\mathcal{C}}
\def\id{{\it I\! d}}
\def\opposite{^{\rm op}}
\def\oddex#1#2{\left\{#1\right\}_{o}^{#2}}
\def\comp#1{{\rm C}^{(#1)}}
\def\ro{\varrho}
\def\ti{-\allowhyphens}
\def\lra{\longrightarrow}

\def\Homeo{\operatorname{Homeo}}
\def\Diff{\operatorname{Diff}}
\def\fix{{\operatorname{Fix}}}
\def\Mat{{\operatorname{Mat}}}
\def\Mod{{\bf Mod}}
\def\zent{{\operatorname{Zent}}}
\def\sym{{\operatorname{Sym}}}
\def\stab{{\operatorname{Stab}}}
\def\arg{{\operatorname{arg}}}
\def\HTP{{\operatorname{HTP}}}
\def\h2{{\operatorname{H_2}}}
\def\h1{{\operatorname{H_1}}}
\def\pr{{\operatorname{pr}}}
\def\rk{{\operatorname{r}}}
\def\tr{{\operatorname{tr}}}
\def\Tr{{\operatorname{Tr}}}
\def\codim{{\operatorname{codim}}}
\def\nt{{\operatorname{nt}}}
\def\d{{\operatorname{d}}}
\def\Gr{{\operatorname{Gr}}}
\def\id{{\operatorname{Id}}}
\def\ker{{\operatorname{ker}}}
\def\im{{\operatorname{im}}}
\def\rot{{\operatorname{Rot}}}
\def\rep{{\operatorname{Rep}}}
\def\Sp{{\operatorname{Sp}}}
\def\PU{{\operatorname{PU}}}
\def\PSL{{\operatorname{PSL}}}
\def\ad{\operatorname{ad}}
\def\Ad{\operatorname{Ad}}
\def\adg{\operatorname{ad}_\frakg}
\def\adp{\operatorname{ad}_\frakp}
\def\det{{\operatorname{det}}}
\def\deta{{\operatorname{det}_A}}
\def\diag{{\operatorname{diag}}}
\def\hom{\operatorname{Hom}}
\def\I{\operatorname{I}}
\def\isp{\operatorname{Is}_{\<\cdot,\cdot\>}}
\def\isptwo{\operatorname{Is}_{\<\cdot,\cdot\>}^{(2)}}
\def\ispth{\operatorname{Is}_{\<\cdot,\cdot\>}^{(3)}}
\def\isf{\operatorname{Is}_F}
\def\isfi{\operatorname{Is}_{F_i}}
\def\isft{\operatorname{Is}_F^{(3)}}
\def\isfit{\operatorname{Is}_{F_i}^{(3)}}
\def\isftwo{\operatorname{Is}_F^{(2)}}
\def\lin{\operatorname{Lin}(L_+,L_-)}
\def\r{\operatorname{r}}
\def\Iso{\operatorname{Iso}}
\def\val{\operatorname{Val}}
\def\Sm{\operatorname{Sm}}
\def\diam{\operatorname{diam}}

\def\bg{B_\frakg}
\def\creg{C_{\rm reg}}
\def\c{\operatorname{c}}
\def\C{{\mathrm{C}}}
\def\cs{\check S}
\def\cst{{\check S}^{(3)}}
\def\gmodp{\gG(\RR)/\pP(\RR)}
\def\gmodq{\gG(\RR)/\qQ(\RR)}
\def\gr{{\rm g}_\RR^*}
\def\grs{{\rm g}_\RR^{(\Sigma,\star)}}
\def\gz{{\rm g}_\ZZ^*}
\def\gzs{{\rm g}_\ZZ^{(\Sigma,\star)}}
\def\ll{{\Ll_1,\Ll_2}}
\def\k{\kappa}
\def\kahler{ K\"ahler }
\def\kbr{\kappa_\RR^b}
\def\kbz{\kappa_\ZZ^b}
\def\kd{\kappa_\DD}
\def\kdb{\kappa_\DD^{\rm b}}
\def\kg{\kappa_G}
\def\kgb{\kappa_{G,\mathrm{B}}}
\def\kgbb{\kappa_{G,\mathrm{B}}^{\rm b}}
\def\kgjb{\kappa_{G,J}^{\rm b}}
\def\kgz{\kappa_{G,\ZZ}}
\def\kgbz{\kappa_{G,\ZZ}^{\rm b}}
\def\kib{\kappa_i^{\rm b}}
\def\kibt{\tilde\kappa_i^{\rm b}}
\def\klb{\k_L^\mathrm{b}}
\def\kljb{\kappa_{L,J}^{\rm b}}
\def\kr{\kappa_\RR}
\def\krlb{\kappa_{\RR,L}^\mathrm{b}}
\def\ku{\kappa_u}
\def\kub{\kappa^{\rm b}_u}
\def\kubr{\kappa_{u,\RR}^{\rm b}}
\def\kubz{\kappa_{u,\ZZ}^{\rm b}}
\def\kur{\kappa_{u,\RR}}
\def\kuz{\kappa_{u,\ZZ}}
\def\kx{\kappa_\Xx}
\def\kxb{\kappa_\Xx^{\rm b}}
\def\kyb{\kappa_\Yy^{\rm b}}
\def\kz{\kappa_\ZZ}

\def\oc{\overline c}
\def\om{\overline m}
\def\oG{\overline G}
\def\pii{\pi_i}
\def\piit{\tilde\pi_i}
\def\psupq{{\rm PSU}(p,q)}
\def\psuvi{{\rm PSU}\big(V,\<\cdot,\cdot\>_i\big)}
\def\rg{r_G}
\def\rhoba{\rho_\mathrm{b}^\ast}
\def\rast{\rho^\ast}
\def\PSU{\mathrm{PSU}}
\def\slv{{\rm SL}(V)}
\def\supq{{\rm SU}(p,q)}
\def\suv{{\rm SU}\big(V,\<\cdot,\cdot\>\big)}
\def\suvi{{\rm SU}\big(V,\<\cdot,\cdot\>_i\big)}
\def\jm{J^{(m)}}
\def\vc{V_\CC}
\def\vconj{\overline v}
\def\wconj{\overline w}

\def\binfty{\mathcal B^\infty_{\mathrm {alt}}}
\def\hcb{{\rm H}_{\rm cb}}
\def\to{\rightarrow}
\def\bu{\bullet}
\def\la{L^\infty_{\mathrm{alt}}}
\def\hb{{\rm H}_{\rm b}}
\def\hc{{\rm H}_{\rm c}}
\def\h{{\rm H}}


\def\sk{\mathsf k}
\renewcommand{\phi}{\varphi}

\def\eI{{^{I}\!\mathrm{E}}}
\def\eII{{^{I\!I}\!\mathrm{E}}}
\def\dI{{^{I}\!d}}
\def\dII{{^{I\!I}\!d}}
\def\fI{{^{I}\!F}}
\def\fII{{^{I\!I}\!F}}

\def\ind{\mathbf{i}}
\def\Ind{\mathrm{Ind}}
\def\No{N\raise4pt\hbox{\tiny o}\kern+.2em}
\def\no{n\raise4pt\hbox{\tiny o}\kern+.2em}
\def\bsl{\backslash}
%
%
%
%
%%%%%%%%%%%%%% Definitionen von Matrizen, etc. %%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mat}[4]{
\left(
\begin{array}{cc}
{\scriptstyle #1} & {\scriptstyle #2} \\ {\scriptstyle #3} & {\scriptstyle
#4}
\end{array}\right)}

\newcommand{\matt}[6]{
\left(
\begin{array}{cc}
{\scriptstyle #1} & {\scriptstyle #2} \\ {\scriptstyle #3} & {\scriptstyle
#4}\\{\scriptstyle #5} & {\scriptstyle #6}
\end{array}\right)}

%\newcommand{\mattt}[16]{
%\left(
%\begin{array}{cccc}
% {\scriptstyle #1} & {\scriptstyle #2} & {\scriptstyle #3} & {\scriptstyle
%#4}\\
%{\scriptstyle #5} & {\scriptstyle #6} & {\scriptstyle #7} & {\scriptstyle
%#8}\\
% {\scriptstyle #9} & {\scriptstyle #{10}} & {\scriptstyle #{11}} & {\scriptstyle
%#{12}}\\
% {\scriptstyle #{13}} & {\scriptstyle #{14}} & {\scriptstyle #{15}} & {\scriptstyle
%#{16}}
%\end{array}\right)}

%\newcommand{\be}[3]{{\beta(y_{#1},y_{#2},y_{#3})}}
\newcommand{\db}[4]{0=d\beta(y_{#1},y_{#2},y_{#3},y_{#4})
= \beta(y_{#1},y_{#2},y_{#3})+\beta(y_{#1},y_{#3},y_{#4})-\beta(y_{#1},y_{#2},y_{#4})
-\beta(y_{#2},y_{#3},y_{#4})}
%
%
%
%


!DSPAM:4696a1d5189941140720403!

